Optimal Ground Station Selection for Low-Earth Orbiting Satellites

This paper presents a solution to the problem of optimal ground station selection for low-Earth orbiting (LEO) space missions that enables mission operators to precisely design their ground segment performance and costs. Space mission operators are increasingly turning to Ground-Station-as-a-Service (GSaaS) providers to supply the terrestrial communications segment to reduce costs and increase network size. However, this approach leads to a new challenge of selecting the optimal service providers and station locations for a given mission. We consider the problem of ground station selection as an optimization problem and present a general solution framework that allows mission designers to set their overall optimization objective and constrain key mission performance variables such as total data downlink, total mission cost, recurring operational cost, and maximum communications time-gap. We solve the problem using integer programming (IP). To address computational scaling challenges, we introduce a surrogate optimization approach where the optimal station selection is determined based on solving the problem over a reduced time domain. Two different IP formulations are evaluated using randomized selections of LEO satellites of varying constellation sizes. We consider the networks of the commercial GSaaS providers Atlas Space Operations, Amazon Web Services (AWS) Ground Station, Azure Orbital Ground Station, Kongsberg Satellite Services (KSAT), Leaf Space, and Viasat Real-Time Earth. We compare our results against standard operational practices of integrating with one or two primary ground station providers.

==> sections/problem_variations.tex <==
\section{Problem Variations}
\label{sec:problem_variations}

We consider three primary variations of the ground station optimization problem. These variations each utilize the objectives and constraints defined in \Cref{sec:ip_formulation}.

\subsection{Mission Cost Minimization Problem}

The mission cost minimization problem variation seeks to minimize the total cost of the ground station network over the mission duration, while also enforcing a minimum per-satellite data downlink requirement is met. The problem formulation also includes \textit{station contact exclusion} and \textit{satellite contact exclusion} constraints. A minimum contact duration constraint is also included to ensure only contacts of at least $t_{min} = $\SI{180}{\s}. The minimum per-satellite constraint is required to ensure a non-degenerate solution, as utilizing no locations, and no providers will otherwise always result in zero cost.

The full optimization problem is
\begin{equation}
\begin{aligned}
   	& \underset{\mathbf{x,l,p,s}}{\text{minimize}} && \sum_{p \in P}C^p_{integ}p \, + \, \sum_{p \in P}\sum_{l \in L^p}C^{p,l}_{setup}l \, + \\
    & &&\, \frac{12 \times T_{opt}}{365.25 \times 86400 \times T_{sim}}\sum_{p \in P}\sum_{l \in L^p}C^{p,l}_{monthly}l \, + \\
    & &&\, \sum_{p \in P}\sum_{l \in L^p}\sum^{|S|}_{i=0} C^{p,l}_{license}v^{p,l}_i \, + \\
    & &&\, \frac{T_{opt}}{T_{sim}}\sum_{p \in P}\sum_{l \in L^p}\sum^{|X^{p,l}|}_{i=0}(C^{p,l}_{pass}t^{p,l}_{pass,i} + C^{p,l}_{pass})x^{p,l}_i \\
    &\text{subject to} && \sum_i^{|X^{p,l}|}x^{p,l}_i = l, \; \forall \; l \in L, p \in P \\
    & && \sum_{l \in L^p}l = p, \; \forall \; p \in P \\
    & && \sum_i^{|X^{p,l,s}|}x^{p,l,s}_i = v^{p,l}, \; \forall \; l \in L, p \in P, v \in S \\
    & && \sum_i^{|X^{p,l}|}\textsc{min}(d_s,d_l)t^{p,l}_{pass,i}x^{p,l}_{i,s} \geq D^v_{min} \; \forall \, i, l, p \; \text{s.t.} \\
   	& && x^{p,l}_{i,s} \in X^{p,l}_s\\
   	& && t^i_{start} \leq t^{window}_{end} \\
   	& && t^i_{end} \geq t^{window}_{start} \\
   	& && t^{window}_{end} = t^{window}_{start} + T^{period} \\
   	& && t^{window}_{start} \in \{t^s_{sim},t^s_{sim}+t_{step},\ldots,t^e_{sim}-T^{period}\} \\
   	& && x^{l,p}_i + x^{l,p}_j \leq 1 \; \forall \; i,j \; \text{s.t.} \\
   	& && t^i_{start} \leq t^j_{end} \\
   	& && t^j_{start} \leq t^i_{end} \\
    & && x^s_i + x^s_j \leq 1 \; \forall \; i,j \; \text{s.t.} \\
   	& && t^i_{start} \leq t^j_{end} \\
   	& && t^j_{start} \leq t^i_{end} \\
   	& && x_i = 0 \; \text{if} \\
   	& && t^i_{end} - t^i_{start} < t_{min} \\
   	& && \sum_i^{|X^{p,l,s}|}\textsc{min}(d-s,d_l)t^{p,l,s}_{pass,i}x^{p,l}_{i,s} \geq D^s_{min}, \\
   	& && \hspace{4cm} \forall \, s \in S, l \in L, p \in P \; \text{s.t.} \\
   	& && t_{start,i} \leq t^{window}_{end} \\
   	& && t_{end,i} \geq t^{window}_{start} \\
   	& && t^{window}_{end} = t^{window}_{start} + T^{period} \\
   	& && t^{window}_{start} \in \{t^s_{sim},t^s_{sim}+t_{step},\ldots,t^e_{sim}-T^{period}\}
\end{aligned}
\label{eqn:prob_min_cost}
\end{equation}

\subsection{Data Volume Maximization Problem}

The mission data maximization problem seeks to maximize the total amount of data downlinked over the mission, while also enforcing a maximum operational cost constraint is met. The problem formulation also includes \textit{station contact exclusion} and \textit{satellite contact exclusion} constraints. A minimum contact duration constraint is also included to ensure only contacts of at least $t_{min} = $\SI{180}{\s}. The maximum operational cost constraint is required to ensure that the optimizer does not simply select all providers and locations to provide the most potential downlink opportunities resulting in a degenerate solution.
\begin{equation}
\begin{aligned}
   	& \underset{\mathbf{x,l,p,s}}{\text{minimize}} && \frac{T_{opt}}{T_{sim}}\sum_{p \in P}\sum_{l \in L^p}\sum^{|X^{p,l}|}_{i=0}\textsc{min}(d_s,d_l)t^{p,l}_{pass,i}x^{p,l}_i \\
   	&\text{subject to} && \sum_i^{|X^{p,l}|}x^{p,l}_i = l, \; \forall \; l \in L, p \in P \\
    & && \sum_{l \in L^p}l = p, \; \forall \; p \in P \\
    & && \sum_i^{|X^{p,l,s}|}x^{p,l,s}_i = v^{p,l}, \; \forall \; l \in L, p \in P, s \in S \\
    & && \frac{365.25 \times 86400}{12T_{sim}} \times \\
    & && \sum_{p \in P}\sum_{l \in L^p}\sum^{|X^{p,l}|}_{i=0}(C^{p,l}_{pass}t^{p,l}_{pass,i} + C^{p,l}_{pass})x^{p,l}_i \, + \\
    & && \sum_{p \in P}\sum_{l \in L^p}C^{p,l}_{monthly}l \, \leq C_{max} \\
   	& && x^{l,p}_i + x^{l,p}_j \leq 1 \; \forall \; i,j \; \text{s.t.} \\
   	& && t^i_{start} \leq t^j_{end} \\
   	& && t^j_{start} \leq t^i_{end} \\
    & && x^s_i + x^s_j \leq 1 \; \forall \; i,j \; \text{s.t.} \\
   	& && t^i_{start} \leq t^j_{end} \\
   	& && t^j_{start} \leq t^i_{end} \\
   	& &&  x_i = 0 \; \text{if} \\
   	& && t^i_{end} - t^i_{start} < t_{min}
\end{aligned}
\label{eqn:prob_min_cost}
\end{equation}

\subsection{Maximum Communications Gap Minimization Problem}

The problem of minimizing the maximum communications gap is the final problem variation. This problem variation represents the design optimization study of a performance-oriented mission design that seeks to minimize communications gaps subject to station exclusion, satellite exclusion, and minimum contact duration constraints.
\begin{equation}
\begin{aligned}
    &\underset{\mathbf{x}}{\text{minimize}} && G_{max} \\ 
    &\text{subject to} && \sum^{|X^{v}|}_{j>i}y_{i,j} = x^{v}_i, \forall i \in |X^{v}|, v \in S \\
    & && (t_{start}^{j} - t_{end}^i)y_{i,j} \leq G_{max}, \; \forall i,j \\
    & && y_{i,j} \leq x^s_i, \; \forall i,j \\
    & && y_{i,j} \leq x^s_j, \; \forall i,j \\
    & && y_{i,j} \in \{0,1\}, \; \forall i,j \\
    & && x^v_i \in \{0,1\}, \; \forall i \\
   	& && x^{l,p}_i + x^{l,p}_j \leq 1 \; \forall \; i,j \; \text{s.t.} \\
   	& && t^i_{start} \leq t^j_{end} \\
   	& && t^j_{start} \leq t^i_{end} \\
    & && x^s_i + x^s_j \leq 1 \; \forall \; i,j \; \text{s.t.} \\
   	& && t^i_{start} \leq t^j_{end} \\
   	& && t^j_{start} \leq t^i_{end} \\
   	& && x_i = 0 \; \text{if} \\
   	& && t^i_{end} - t^i_{start} < t_{min}
\end{aligned}
\label{eqn:prob_min_max_gap}
\end{equation}
